AGRO: Adversarial Discovery of Error-prone groups for Robust Optimization

Models trained via empirical risk minimization (ERM) are known to rely on spurious correlations between labels and task-independent input features, resulting in poor generalization to distributional shifts. Group distributionally robust optimization (G-DRO) can alleviate this problem by minimizing the worst-case loss over a set of pre-defined groups over training data. G-DRO successfully improves performance of the worst-group, where the correlation does not hold. However, G-DRO assumes that the spurious correlations and associated worst groups are known in advance, making it challenging to apply it to new tasks with potentially multiple unknown spurious correlations. We propose AGRO -- Adversarial Group discovery for Distributionally Robust Optimization -- an end-to-end approach that jointly identifies error-prone groups and improves accuracy on them. AGRO equips G-DRO with an adversarial slicing model to find a group assignment for training examples which maximizes worst-case loss over the discovered groups. On the WILDS benchmark, AGRO results in 8% higher model performance on average on known worst-groups, compared to prior group discovery approaches used with G-DRO. AGRO also improves out-of-distribution performance on SST2, QQP, and MS-COCO -- datasets where potential spurious correlations are as yet uncharacterized. Human evaluation of ARGO groups shows that they contain well-defined, yet previously unstudied spurious correlations that lead to model errors.

==> sections/contributions.tex <==
\begin{itemize}
    \item AGRO optimization framework --- An end-to-end framework to both, identify slices in the training data with potential spurious-attributes and train a model that is robust to the identified worst groups. Note - unlike all prior work that makes some assumptions about the knowledge of spurious attributes (in the dev set), we make no such assumptions at all. We are solving this problem with the fewest assumptions about what is spurious and what is not.  
    \item AGRO adversary features --- Prior work that has attempted to discover slices for group robustness have relied on learned representations and loss of the ERM model. We take inspiration from two recent advances - a)  representation learning via pre-training that is less prone to learn dataset-specific short-cuts and b) training dynamics of the ERM model which provides information about how a particular example is learned over the course of training that can correlate with the existence of short-cuts in the example. Empirically, we find that these these additional features, while being task-agnostic, are useful for the slice discovery problem. 
    \item Model selection (1 sentence) --- Prior work like JTT, EIIL still require knowledge of the spurious attribute on a small development set during model selection. We work in an even harder setting where that is not available (for datasets like SST-2, ImageNet, Bool-Q and QQP), instead relying on the slices discovered by AGRO for model selection. We find that even in that case, we are able to show improved robustness to distributional shifts. This allows for AGRO to be used on any new dataset to build a model that is robust to distributional shifts in the training data. 
    \item Other minor contributions - With AGRO, we allow for soft grouping which is useful when multiple attributes may be active in a given example.
\end{itemize}
